Beyond the Hype: A Comprehensive Review of Current Trends in Generative AI Research, Teaching Practices, and Tools

Generative AI (GenAI) is advancing rapidly, and the literature in computing education is expanding almost as quickly. Initial responses to GenAI tools were mixed between panic and utopian optimism. Many were fast to point out the opportunities and challenges of GenAI. Researchers reported that these new tools are capable of solving most introductory programming tasks and are causing disruptions throughout the curriculum. These tools can write and explain code, enhance error messages, create resources for instructors, and even provide feedback and help for students like a traditional teaching assistant. In 2024, new research started to emerge on the effects of GenAI usage in the computing classroom. These new data involve the use of GenAI to support classroom instruction at scale and to teach students how to code with GenAI. In support of the former, a new class of tools is emerging that can provide personalized feedback to students on their programming assignments or teach both programming and prompting skills at the same time. With the literature expanding so rapidly, this report aims to summarize and explain what is happening on the ground in computing classrooms. We provide a systematic literature review; a survey of educators and industry professionals; and interviews with educators using GenAI in their courses, educators studying GenAI, and researchers who create GenAI tools to support computing education. The triangulation of these methods and data sources expands the understanding of GenAI usage and perceptions at this critical moment for our community.

==> EduDevViews.tex <==
Our surveys and interviews sought to gather a wider perspective on how Generative AI and large language models change the way software is developed and how instructors' teaching changes or will change:


\subsection{Methods}
\subsubsection{Research Questions}
\input{EduDevViews-methods}

\subsubsection{Methods---Survey}
\input{survey-methods}

\subsubsection{Methods---interview}
\input{interview-method}

\subsection{Results}
\input{EduDevViews-results}



==> interview-method.tex <==









\subsection{Interviews}
We compiled a list of individuals who fit into one  of the following three categories:\\
\begin{itemize}
    \item Tool creators,
    \item Educators studying GenAI, and
    \item Educators using GenAI.
\end{itemize}

The interviewees have been active in the computing education community in one or more of the areas identified above. The research team completed X, Y, and Z interviews in each of the respective areas above. 

We created research questions to aid in our pursuit of our overall research goals. Therefore, each of the following research questions links back to our overarching research goals. We used these research questions to guide our analysis of the transcripts:

We seek to answer the following questions:
\begin{itemize}
    \item \textbf{Instruction-use:} How are instructors teaching students about using generative AI tools in order to program? e.\,g. Promptly (1a)
    \item \textbf{Instruction-support:} How are instructors using generative AI tools to support the teaching of their courses? E.\,g. grading, chatbot (CS50, CodeHelp, CodeAid), feedback, assignment creation, anything “learning with the tool” (1a)
    \item \textbf{Tools:} What kinds of GenAI tools are emerging in computing education? (1a)
    \item \textbf{Policies:} What are the existing policies and practices around using GenAI in computing courses? (1b)
    \item \textbf{Motivations:} Why are instructors making these choices around using GenAI? (1b)
    \item \textbf{Competencies:} How has GenAI impacted desired student competencies? (2a, 2b)
    \item \textbf{Outcomes:} How has GenAI impacted actual student outcomes (compared to before)? (2a)
    \item \textbf{Industry usage:} How are industry developers using GenAI tools? (2a)
    \item \textbf{Future:} How is GenAI shaping the future of computing education? (2b)
\end{itemize}



==> interview-results.tex <==
\section{Interviews}
Intro to results here with callback to our RQs.


\subsection{Instruction-use}
% How are instructors teaching students about using generative AI tools in order to program? e.g. Promptly (1a)

\subsection{Instruction-support}
% How are instructors using generative AI tools to support the teaching of their courses? E.g. grading, chatbot (CS50, CodeHelp, CodeAid), feedback, assignment creation, anything “learning with the tool” (1a)

\subsection{Tools}
%What kinds of GenAI tools are emerging in computing education? (1a)

\subsection{Policies}
%What are the existing policies and practices around using GenAI in computing courses? (1b)

\subsection{Motivations} %formerly: "Why Policies"
%Why are instructors making these choices around using GenAI? (1b)

\subsection{Competencies}
%How has GenAI impacted desired student competencies? (2a, 2b)

\subsection{Outcomes}
%How has GenAI impacted actual student outcomes (compared to before)? (2a)

\subsection{Industry usage}
%How are industry developers using GenAI tools? (2a)

\subsection{Equity}
%How has GenAI impacted student equity?

\subsection{Future}
%How is GenAI shaping the future of computing education? (2b)
